A polyconvex transversely-isotropic invariant-based formulation for electro-mechanics: stability, minimisers and computational implementation

The fabrication of evermore sophisticated miniaturised soft robotic components made up of Electro-Active Polymers (EAPs) is constantly demanding parallel development from the in-silico simulation point of view. The incorporation of crystallographic anisotropic micro-architectures, within an otherwise nearly uniform isotropic soft polymer matrix, has shown great potential in terms of advanced three-dimensional actuation (i.e. stretching, bending, twisting), especially at large strains, that is, beyond the onset of geometrical pull-in instabilities. To accommodate for this in-silico response, this paper presents a phenomenological invariant-based polyconvex transversely isotropic framework for the simulation of EAPs at large strains. This research expands previous work developed by Gil and Ortigosa for isotropic EAPs with the help of the pioneering work by Schr\"{o}eder and Neff in the context of polyconvexity for materials endowed with crystallographic architectures in single physics mechanics. The paper also summarises key important results both in terms of the existence of minimisers and material stability. In addition, a series of numerical examples is presented in order to demonstrate the effect that the anisotropic orientation and the contrast of material properties, as well as the level of deformation and electric field, have upon the response of the EAP when subjected to large three-dimensional stretching, bending and torsion, including the possible development of wrinkling.

==> sections/FEM.tex <==
Here, we focus only on a formulation based on three field formulation, introduced in \cite{gil2016new}, with displacements, electric field, and electric displacement as the primary variables.
The energy of the system is expressed as
\begin{equation}\label{eq:HW_functional}
\mathcal{E}(\bm{y},\varphi, \bm{D}_0):=\int_\O W(\bm{\nabla} \bm{y}(\bm{x}),\bm{D}_0(\bm{x}))\,\md x +\int_\O \bm{\nabla}\varphi(\bm{x})\cdot\bm{D}_0(\bm{x})\,\md x-L(\bm{y}(\bm{x}),\varphi)
\end{equation}
The stationary conditions of the above functional (\ref{eq:HW_functional}) yields  
\begin{eqnarray}\label{eq:StationarityHu-Washizu}
D{\mathcal{E}}[\delta \bm{u}, \delta {\varphi}, \delta \bm{D}_0]=
\int_{\Omega} \left(\frac{\partial W}{\partial \bm{F}}:\bm{\nabla}\delta \bm{u} + \frac{\partial W}{\partial \bm{D}_0}\cdot\delta \bm{D}_0 + \bm{\nabla}\delta\varphi\cdot \bm{D}_0 + \bm{\nabla}\varphi\cdot\delta\bm{D}_0\right)\,\md \bm{x} - D L[\delta\bm{y}(\bm{x}), \delta\varphi]  = \bm{0}\nonumber
\end{eqnarray}
{\mh
with $\bm{u}\in V^u$, $\varphi \in V^\varphi$, $\bm{D}_0 \in V^D$, and with the admissible variations $\delta \bm{u} \in V^u_0$, $\delta \varphi \in V^\varphi_0$, and $\delta \bm{D}_0 \in V^D$
where
\begin{eqnarray}
\nonumber
V^{u} &=&\begin{Bmatrix}\bm{u}:\O_0\rightarrow\R^3;\; \bm{u}\in H^1(\O_0)\;\vert\; \bm{u} = \bar{\bm{u}}\;\text{on}\; \partial\O_0^u  \end{Bmatrix} \quad V_0^{u} =\begin{Bmatrix}\bm{u}:\O_0\rightarrow\R^3;\; \bm{u}\in H^1(\O_0)\;\vert\; \bm{u} = \bm{0} \;{\text on}\; \partial\O_0^u  \end{Bmatrix}
\\
\nonumber
V^{{\varphi}} &=&\begin{Bmatrix}{\varphi}:\O_0\rightarrow\R;\; {\varphi}\in H^1(\O_0)\;\vert\; {\varphi} = \bar{{\varphi}} \;{\text on}\; \partial\O_0^\varphi  \end{Bmatrix}
\quad
\;\;
V_0^{{\varphi}} =\begin{Bmatrix}{\varphi}:\O_0\rightarrow\R;\; {\varphi}\in H^1(\O_0)\;\vert\; {\varphi} = 0 \;{\text on}\; \partial\O_0^\varphi  \end{Bmatrix}
\\
\nonumber
V^{D}&=&\begin{Bmatrix}\bm{D}_0:\O_0\rightarrow\R^3;\; \bm{D}_0\in L_2(\O_0) \end{Bmatrix}
\end{eqnarray}

It is worth emphasizing that the stationarity condition (\ref{eq:StationarityHu-Washizu}) corresponds to the weak forms of
}
\begin{itemize}
    \item conservation of linear momentum
    \begin{eqnarray}\label{eq:WeakMomentum}
    \int_{\Omega} \frac{\partial W}{\partial \bm{F}}:\bm{\nabla}\delta \bm{u}  - D L[\delta \bm{y}(\bm{x})] = 0
    \end{eqnarray}
    \item Gauss's law
    \begin{eqnarray}\label{eq:WeakGauss}
    \int_{\Omega}  \bm{\nabla}\delta\varphi\cdot \bm{D}_0 \,\md \bm{x} - D L[\delta \varphi] = 0
\end{eqnarray}
\item Faraday's law
    \begin{eqnarray}\label{eq:WeakFaraday}
    \int_{\Omega}\left(\frac{\partial W}{\partial \bm{D}_0} + \bm{\nabla}\varphi\right)\cdot\delta \bm{D}_0\,\md \bm{x} = 0
    \end{eqnarray}
\end{itemize}
where
\begin{eqnarray}
D L[\delta \bm{y}(\bm{x})] &=& - \int_\Omega \bm{b}\cdot\delta\bm{u}\; {\rm d}\bm{x} - \int_{\partial\Omega_t} \bar{\bm{T}}\cdot\delta\bm{u}\; {\rm d}{\Gamma}
\\
D L[\delta \varphi] &=& - \int_{\Omega} \bm{\rho}^e_0 \delta\varphi\; {\rm d}\bm{x}- \int_{\delta\Omega_\omega} \bm{\omega}^e_0 \delta\varphi\; {\rm d}\bm{\Gamma} 
\end{eqnarray}
are the virtual work of external forces and external work contribution due to the electrical effects.

Further, we apply the standard isoparametric finite elements. Thus, {\mh the domain $\O_0$ is divided into elements and }the displacements, electric potential, and electric displacements {\mh are approximated by means of approximation finite element spaces $V^u_h \subset V^u$, $V^\varphi_h \subset V^\varphi$, and $V^D_h \subset V^D$ defined as
\begin{eqnarray}
\nonumber
V_h^{u} &=&\begin{Bmatrix}\bm{u}:\O_0\rightarrow\R^3;\; \bm{u} = \sum_{a=1}^{n^u_{nod}}N_u^a d^a_u\;\vert\; \bm{u} = \bar{\bm{u}}\;{\rm on}\; \partial\O_0^u  \end{Bmatrix} \\
\nonumber
V_h^{\varphi} &=&\begin{Bmatrix}{\varphi}:\O_0\rightarrow\R^3;\; \varphi = \sum_{a=1}^{n^\varphi_{nod}}N_\varphi^a d^a_\varphi\;\vert\; \varphi = \bar{\varphi}\;{\rm on}\; \partial\O_0^\varphi  \end{Bmatrix}
\\
\nonumber
V_h^{D}&=&\begin{Bmatrix}\bm{D}_0:\O_0\rightarrow\R^3;\; \bm{D}_0= \sum_{a=1}^{n^D_{nod}}N_D^a d^a_D \end{Bmatrix}
\end{eqnarray}
where for any field $i = \begin{Bmatrix}{{u},\varphi,D}\end{Bmatrix}$, $n^i_{nod}$ denotes number of the appropriate element nodes, $N_i^a$ is the $a$-th basis function, and $\bm{d}_i^a$ is the $a$-th nodal degree of freedom of the appropriate field.
Denoting $\bm{N}_i$ matrices collecting the finite element interpolation functions, and $\bm{d}_i$ vectors collecting the degrees of freedom, we can write
}
\begin{eqnarray}\label{eq:FEM_discr}
\bm{u} = \bm{N}_u \bm{d}_u \qquad
{\varphi} = \bm{N}_\varphi \bm{d}_\varphi 
\qquad 
\bm{D}_0 = \bm{N}_D \bm{d}_D
\end{eqnarray}
Moreover, the displacement gradient and gradient of the electric potential are written as
\begin{eqnarray}\label{eq:FEM_discrGrad}
\bm{\nabla}_0\bm{u} = \bm{B}_u \bm{d}_u
\quad \bm{\nabla}_0\varphi = \bm{B}_\varphi \bm{d}_\varphi
\end{eqnarray}
where $\bm{B}_i$ are matrices collecting the derivatives of the finite element interpolation functions. Note that the Bubnov-Galerkin approach is assumed, i.e., the variations $\delta \bm{u}$, $\delta \varphi$, $\delta \bm{D}_0$, and the gradients $\bm{\nabla}_0\delta \bm{u}$, $\bm{\nabla}_0\delta \varphi$ are approximated in analogy with (\ref{eq:FEM_discr}) -- (\ref{eq:FEM_discrGrad}).

Substituting these relations into (\ref{eq:WeakMomentum})--(\ref{eq:WeakFaraday}), we arrive at a set of nonlinear equations to be solved
\begin{equation}
\bm{f}_{int}(\bm{d}) =  \bm{f}_{ext}  
\end{equation}
with $\bm{d} = \begin{bmatrix}\bm{d}_u, \bm{d}_\varphi, \bm{d}_D\end{bmatrix}^T$, $\bm{f}_{int}  = \begin{bmatrix}\bm{f}^u_{int}, \bm{f}^\varphi_{int}, \bm{f}^D_{int}\end{bmatrix}^T$, and $\bm{f}_{ext}  = \begin{bmatrix}\bm{f}^u_{ext}, \bm{f}^\varphi_{ext}, \bm{0}\end{bmatrix}^T$,
denoting vectors of generalized degrees of freedom, generalized internal forces, and generalized external forces, where the individual components are given as
\begin{eqnarray}
\bm{f}^u_{int} &=& \int_{\Omega_0} \bm{B}^T_u \bm{P} \; {\rm d}V \qquad
\bm{f}^\varphi_{int} = \int_{\Omega_0} \bm{B}^T_\varphi  \bm{D}_0 \; {\rm d}V \qquad
\bm{f}^D_{int} = \int_{\Omega_0} \bm{N}_D^T\left( \bm{E} + \bm{\nabla}\varphi\right) \; {\rm d}V 
\\
\bm{f}_{ext}^u &=&  \int_{\Omega_0} \bm{N}^T_u\bm{b}\; {\rm d}\bm{x} + \int_{\partial_{\Omega^t_0}} \bm{N}^T_u\bar{\bm{t}}\; {\rm d}{\Gamma}
\qquad
\bm{f}_{ext}^\varphi =  \int_{\Omega_0} \bm{N}^T_\varphi \bm{\rho}^e_0 \delta\varphi\; {\rm d}\bm{x}+ \int_{\delta\Omega_0^\omega} \bm{N}^T_\varphi\bm{\omega}^e\; {\rm d}\bm{\Gamma} 
\end{eqnarray}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
To express the Hessian matrix, linearization of the stationary condition (\ref{eq:StationarityHu-Washizu}) is exploited as
\begin{eqnarray}\label{eq:StationarityHu-Washizu}
\nonumber
D^2{\mathcal{E}}[\delta \bm{u}, \delta {\varphi}, \delta \bm{D}_0;\Delta \bm{u}, \Delta {\varphi}, \Delta \bm{D}_0] = \int_{\Omega_0} \bm{\nabla}_0\Delta\bm{u}:\frac{\partial^2 W}{\partial \bm{F}\partial \bm{F}}:\bm{\nabla}_0\delta \bm{u}+\Delta\bm{D}_0:\frac{\partial^2 W}{\partial \bm{F}\partial \bm{D}_0}:\bm{\nabla}_0\delta \bm{u}
\\
+ \Delta \bm{D}_0\cdot\frac{\partial^2 W}{\partial \bm{D}_0\partial \bm{D}_0}\cdot\delta \bm{D}_0 + \bm{\nabla}_0\Delta \bm{u}\cdot\frac{\partial^2 W}{\partial \bm{D}_0\partial \bm{F}}\cdot\Delta \bm{D}_0 + \bm{\nabla}_0\delta\varphi\cdot \Delta\bm{D}_0 + \bm{\nabla}_0\Delta\varphi\cdot\delta\bm{D}_0\,\md V
\end{eqnarray}
leading to the tangent electro-mechanics modulus $\bm{K}$ 
\begin{equation}
D^2{\mathcal{E}}[\delta \bm{u}, \delta {\varphi}, \delta \bm{D}_0;\Delta \bm{u}, \Delta {\varphi}, \Delta \bm{D}_0] = \begin{Bmatrix}
\delta \bm{u}\\ \delta {\varphi}\\ \delta \bm{D}_0
\end{Bmatrix}^T\underbrace{\begin{bmatrix}
\bm{K}_{uu} & \bm{0} & \bm{K}_{uD}\\
\bm{0} & \bm{0} & \bm{K}_{D\varphi}\\
\bm{K}_{Du} & \bm{K}_{\varphi D} & \bm{K}_{DD}
\end{bmatrix}}_{\bm{K}}\begin{Bmatrix}
\Delta \bm{u}\\ \Delta {\varphi}\\ \Delta \bm{D}_0
\end{Bmatrix}
\end{equation}
with individual components defined as
\begin{eqnarray}
\bm{K}_{uu} &=& \int_{\Omega_0} \bm{B}^T_u \frac{\partial^2 W}{\partial \bm{F}\partial \bm{F}} \bm{B}_u\; {\rm d}V 
\qquad
\;\;\;
\bm{K}_{uD} = \int_{\Omega_0} \bm{B}^T_u \frac{\partial^2 W}{\partial \bm{F}\partial \bm{D}_0} \bm{N}_D\; {\rm d}V 
\\
\bm{K}_{Du} &=& \int_{\Omega_0} \bm{N}^T_D \frac{\partial^2 {W}}{\partial \bm{D}_0\partial \bm{F}} \bm{B}_u\; {\rm d}V 
\qquad
\bm{K}_{DD} = \int_{\Omega_0} \bm{N}^T_D \frac{\partial^2 W}{\partial \bm{D}_0\partial \bm{D}_0} \bm{N}_D\; {\rm d}V 
\\
\bm{K}_{\varphi D} &=& \int_{\Omega_0} \bm{B}^T_\varphi \bm{N}_D \; {\rm d}V 
\qquad
\;\;\;\;\;\;\;\;\;\;\;\
\bm{K}_{D \varphi } = \int_{\Omega_0} \bm{N}^T_D \bm{B}_\varphi  \; {\rm d}V 
\end{eqnarray}

